FedComm: Understanding Communication Protocols for Edge-based Federated Learning

Federated learning (FL) trains machine learning (ML) models on devices using locally generated data and exchanges models without transferring raw data to a distant server. This exchange incurs a communication overhead and impacts the performance of FL training. There is limited understanding of how communication protocols specifically contribute to the performance of FL. Such an understanding is essential for selecting the right communication protocol when designing an FL system. This paper presents FedComm, a benchmarking methodology to quantify the impact of optimized application layer protocols, namely Message Queue Telemetry Transport (MQTT), Advanced Message Queuing Protocol (AMQP), and ZeroMQ Message Transport Protocol (ZMTP), and non-optimized application layer protocols, namely as TCP and UDP, on the performance of FL. FedComm measures the overall performance of FL in terms of communication time and accuracy under varying computational and network stress and packet loss rates. Experiments on a lab-based testbed demonstrate that TCP outperforms UDP as a non-optimized application layer protocol with higher accuracy and shorter communication times for 4G and Wi-Fi networks. Optimized application layer protocols such as AMQP, MQTT, and ZMTP outperformed non-optimized application layer protocols in most network conditions, resulting in a 2.5x reduction in communication time compared to TCP while maintaining accuracy. The experimental results enable us to highlight a number of open research issues for further investigation. FedComm is available for download from https://github.com/qub-blesson/FedComm.

==> sections/conclusion.tex <==
In this paper, we proposed \FedComm,\, a benchmarking method for FL application layer protocols. We evaluated the major application layer protocols that could be used in a FL context, such as standard TCP, standard UDP, MQTT, AMQP, and ZMTP. TCP outperformed UDP as a non-optimized application layer protocol in many experiments, with higher accuracy and shorter communication times, especially for smaller models like the VGG-5 in our study. On larger models such as the VGG-8, UDP performed better in terms of communication time. AMQP, as the optimized application layer protocol, outperformed non-optimized TCP in most network conditions. MQTT performed similarly to AMQP, but with faster communication times for smaller model types. The optimised application layer protocols demonstrated high accuracy with minor differences of $<$0.5\% at certain points.

\textit{\textbf{Future Research:}} Currently, \FedComm\ evaluates a limited number of core application layer protocols and highlights the fundamental functionality of each protocol. As a future work, we highlight a number of application layer enhancements within the context of FL that require further investigation.

\textit{Reliable implementation of socket UDP for FL:} We will improve and thoroughly test UDP socket implementation with additional parameters. \FedComm\ will support adjusting the size of UDP chunks, giving users more control over communication time and accuracy. After receiving model weights via UDP that contain erroneous model weights or missing parameters, we will attempt to provide an in-depth analysis of the various methods for filling in the missing values in the model.

\textit{Enhancement of standard MQTT, AMQP and ZMTP for FL:} MQTT will be evaluated using various broker configurations, including both local and public brokers, to provide a more in-depth analysis of real-world MQTT usage. Furthermore, MQTT for sensor networks will be added to \FedComm\ and compared to standard MQTT in the FL setting.

Different brokers will be implemented for AMQP to investigate the differences in how AMQP operates; will communication time be reduced? Will the accuracy improve? Will there be a change in packet loss? All of this will be thoroughly investigated. Moreover, we will attempt to change the architecture of AMQP and investigate how this different architecture will affect AMQP in a FL setting.

ZMTP is highly modifiable; various messaging types will be compared to all application layer protocols, including request/response, pull/push, pipeline, and pairs. To provide a more in-depth evaluation of the application layer protocols in various environments, we will attempt to scale the testbed by adding more devices.

==> sections/metrics.tex <==
In this section, we discuss the performance metrics used to evaluate application and transport layer protocols in FL.


\begin{itemize}[]
	\item \textbf{Accuracy:} {Accuracy is defined as the number of correct predictions divided by the total number of predictions. This metric measures how accurate the new aggregated model is against the test data per FL round.}
	
	\item \textbf{Communication time:} {This metric calculates the total communication time across all FL rounds. The communication time includes the time spent sending and receiving model parameters between devices and server during FL training.}
	
	\item \textbf{Performance under computational stress:} {
	This metric measures the total communication time under computational stress. The Stress-ng~\cite{stressng} module is used to spawn threads to increase the number of computations performed in order to simulate a working networked device. Stress-ng compute 830 ops/s using 99\% of the CPU power to simulate a low-power device incapable of performing large tasks.}
	
	\item \textbf{Performance under network stress:} {This metric measures the total amount of communication time spent under network stress. Netstress emulates an active network, sending messages at around 250 Mbits/s.}
	
	\item \textbf{Packet loss rate or re-transmission rate:} {This metric is used to calculate the packet loss rate for UDP-based protocols by counting the sent and received packets, and the re-transmission rate for TCP-based protocols.}
	

\end{itemize}


==> sections/relatedwork.tex <==
The communication overhead incurred in FL at the edge is well documented in the existing research literature~\cite{wang2019adaptive, 9148862, he2020group}. 
Multiple approaches can be adopted to alleviate this problem. Firstly, developing techniques at the algorithmic level of the application to reduce or limit the volume of data transferred between devices and servers. There is a large body of research that focuses on this approach, which is considered further in this section. For example, numerous compression techniques have emerged that addresses communication efficiency.  

Secondly, developing the underlying techniques, such as at the communication protocol level focused towards FL to make data transmission more efficient. However, there is limited research in this area and, therefore, the focus of this paper is a preliminary step in this direction to quantify the impact of communication protocols in FL.  

Compression techniques reduce the volume of data that is transferred between devices and the server. However, the overall accuracy of the model that is trained using FL is affected. 
A few examples of the compression techniques that have been used in FL are Deep Gradient Compression (DGC)~\cite{46622} and BottleNet~\cite{Eshratifar2019BottleNetAD}. 

The Deep Gradient Compression (DGC)~\cite{46622} technique reduces the volume of data transferred without significantly sacrificing accuracy (only 0.03\% accuracy in some cases). However, this technique requires changes to the ML algorithm, which is akin to reengineering the application and is thus an intrusive approach. 

BottleNet~\cite{Eshratifar2019BottleNetAD}, another compression technique is based on standard JPEG compression. 
The implementation changes required are specific to the input. 

Other techniques, include ScissionTL~\cite{DBLP:journals/corr/abs-2105-02019} and Three Lossy Compression (3LC)~\cite{Lim20193LCLA} that reduce the amount of data transferred while attempting to maintain accuracy.

Additions to compression techniques, such as sparsification, ternarization, error accumulation and optimal Golomb encoding have been developed in STC~\cite{8889996}. These result in a faster convergence rate than FedAvg (the classic algorithm used in FL) but has limited performance in certain scenarios.

RingFed~\cite{Yang2021RingFedRC} reduces communication costs by limiting data transfers between the server and devices. This is achieved by only one device receiving model updates from the server and then passing it on to other clients in a ring fashion. The last device receiving the updates will upload the parameters to the server. One major consideration in such an approach is that the devices need to communicate as peers, which may be less feasible in the real-world. 

Alternate approaches to the above as mentioned previously is to employ lightweight communication protocols, such as MQTT, AMQP, ZMPT, and socket TCP or UDP, or develop new protocols that are suited for FL. However, from the literature there is limited research on the impact of these protocols on FL, which is the focus of this paper. 
